High-Order Attention Models for Visual Question Answering

The quest for algorithms that enable cognitive abilities is an important part of machine learning. A common trait in many recently investigated cognitive-like tasks is that they take into account different data modalities, such as visual and textual input. In this paper we propose a novel and generally applicable form of attention mechanism that learns high-order correlations between various data modalities. We show that high-order correlations effectively direct the appropriate attention to the relevant elements in the different data modalities that are required to solve the joint task. We demonstrate the effectiveness of our high-order attention mechanism on the task of visual question answering (VQA), where we achieve state-of-the-art performance on the standard VQA dataset.

==> intro.tex <==
%!TEX root = nips_2017.tex
\section{Introduction}
%What is the problem and why is it important
Understanding a scene in its entirety is the goal of computer vision. However, achieving this ambitious target turned out to be more difficult than expected. Partly because  holistic scene understanding  requires to capture and take into account information from multiple modalities (\ie, text, image)  on various levels from objects, and actions, to  even general knowledge. The tremendous amount of plausible explanations makes this task extremely demanding~\cite{yao2012describing,DBLP:journals/corr/RenHG015}.

In recent years, significant progress has been reported on a large variety of recognition tasks from object detection to semantic segmentation. However, many of these results focus on solving  isolated problems in a controlled environment. Consider, for example, datasets for object detection, semantic segmentation, action classification \etc. Less of an effort has been devoted to addressing various recognition problems simultaneously, largely because it is a more complex endeavor.


Visual Question Answering (VQA) is one of the tasks which requires more complex reasoning. Answering questions based on images requires knowledge extracted from a variety of recognition tasks at various levels, such as counting objects, detecting colors, but also  understanding the scene, emotional intelligence and general knowledge. In addition, to correctly answer a question, it is require to understand both accurately. Tools which automatically extract this form of understanding from data are very widely applicable and hence of tremendous societal interest.

To address the VQA challenge, present day frameworks first extract image and question features. Image features are typically obtained from deep nets, like VGG~\cite{DBLP:journals/corr/SimonyanZ14a}, pre-trained on classification tasks, like ImageNet~\cite{ILSVRC15}. Question features are obtained from variations of long short-term memory (LSTM) nets~\cite{hochreiter1997long}. An straightforward approach combines the features, either via concatenation, summation or other algebraic operations, and employs a classifier to choose from the top-K answers found in the training set. 
This solution works remarkably  well, but numerous papers have shown that an attention mechanism can improve the results significantly~\cite{DBLP:journals/corr/MalinowskiF14}.  An attention module learns to highlight one or multiple specific regions of interest in the image and in the question, by creating a probability distribution over the corresponding feature space. This probability distribution indicates the importance of a specific pixel or word representation for the answer. Existing algorithms, \eg,~\cite{DBLP:journals/corr/MalinowskiF14}, usually treat the attention mechanism as a single unit modifying the provided features. 

In this paper we argue that this view is problematic, as even the simplest VQA task involves data from multiple modalities, text and image. To design a valuable attention mechanism for such an application, we need to appreciate its multi-modal input and design a multi-variate probability model. Such a more complex probability model is able to better capture the details of the data.

Current techniques usually deal with multi-modality,  by first combining the features of different data types. Afterwards, attention is applied over the combined vector. This approach is less natural and neglects the original concept of attention as a probability distribution.

%How do we propose to solve the problem and why is this better

Therefore, we propose a new form of attention mechanism %{\color{red}inspired from Markov random field} %-- high order attention -- 
constructed from `unary potentials,' based on individual data representations, and  `pairwise potentials,'  based on any combination of two data modalities. %allow the model to learn pairwise potentials by considering the orthogonality of features from two modalities. 
We then use the marginals of the pairwise attention to emphasize the importance of the data representation. In this way we are able to take advantage of the correlations between two different modalities.

Our technique illustrates that attention is an effective and interpretable mechanism to combine multiple data  modalities. Besides, our approach also facilitates further understanding about how different modules work together.
To demonstrate this behavior we show in~\figref{fig:Teaser} the result of our different attention modules as well as the parts of the image and question that our module attends to.

%What do we evaluate it on
We investigate the effectiveness of our method by evaluating our technique on the complex task of visual question answering. VQA is an example for tasks that require multi-modal input, in this case the question and image, which are to be integrated into a single output. Additionally, multiple choice VQA introduce a third modality, \ie, a set of answers, which we use to demonstrate how to use our attention mechanism on three modalities. 




